The peculiar new state of the blazar PKS 1510-089

Contemporaneous multiwavelength observations with H.E.S.S., SALT, Fermi-LAT, Swift, and ATOM show that the blazar PKS 1510-089 suffered a significant decrease in its optical flux, degree of optical polarization and high-energy gamma-ray (E > 100 MeV) flux since July 2021. Meanwhile, the X-ray and very-high-energy gamma-ray (E > 100 GeV) fluxes remained steady throughout 2021 and 2022. The degree of optical polarization decreased to about zero in 2022, indicating an unpolarized dominating accretion disk component in the optical-UV domain that is completely diluting the polarized electron synchrotron component. In this proceeding we will discuss, via theoretical SED modeling, possible reasons for this dramatic change in the appearance of this blazar.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

